Probing the Quantum and Classical Boundary: A Tabletop Experiment Using Quantum Optics

In this work, we propose a simple but effective experiment for probing the boundary in which a wave-function collapses. Using a quantum optics system interacting with a photomultiplier tube (PMT), one is able to determine the number of electrons needed to interfere with the "which-path" information to cause the collapse of a quantum state.

==> docs/discussion.tex <==
\section{Discussion of Potential Results and Implications} 

In section \ref{fig:experiment_diagram}, we have outlined that we want to place different devices for the "measurement" at $D_1$. Now, we discuses the potential results and implications. Recall that we want to focus on 3 different detectors:
\begin{enumerate}
    \item Cold Atom Gas
    \item Photo Multiplier Tube
    \item Photographic Plate
\end{enumerate}
And use the different detector to test for the criteria of causing the state at $D_0$ to collapse. Let us discuss each of these below.

\subsection{Cold Atom Gases}
We start by considering the cold atom gas. Let us assume we have found a good medium with a absorption spectrum compatible with the idler photons. Then, when a idler photon is absorbed, the cold atom gas has essentially "learned" the which path information. This is approximately the following process:
\begin{align}
    \ket{1}_{i, B} \ket{0}_{atom} \longrightarrow \ket{0}_{i, B} \ket{1}_{atom}
\end{align}
One may ask, does this collapse the state at detector $D_0$. The authors believe the answer is no, but it is interesting to see this in experiment. 

\subsection{Photographic Plate}
If the cold atom gas does not cause collapse of the quantum state, we may consider instead placing a photographic plate or film at $D_0$. Physical process of happening at the film is as follows:
\begin{align}
    \text{AgX} + \text{light} \rightarrow \text{Ag} + \text{X}^-
\end{align}
Where $AgX$ represents a silver halide crystal. The sliver halide may be unresponsive to a single photon hit, but repeated bombardment, like in a experimental setting, allows the average locations of the photons to be recorded. It is then interesting to see experimentally if this counts as an measurement of the which-path information. 

\subsection{Photo Multiplier Tube}
The photo multiplier tube is the most interesting case. If the previous "measurements" do not cause the state at $D_0$ to collapse, we may consider using a photomultiplier tube (PMT) to amplify the photons. A photo-multiplier tube utilizes the photo-electric effect to achieve single photon resolution. The physical process goes as follows:

The photon hits a photocathode, which releases a electron (through the photoelectric effect) when the photon hits. A series of dynode is placed afterwards. A voltage is applied, so that the electron accelerates and hits the dynode, and releases more electrons. 

By placing many dynode, the signal is amplified. This amplification is exponential. In a PMT, the total amplification factor is dependent on the number of dynode, or stages of the PMT, and the amplification factor per stage. Let us say that we have a amplification of $G$ per stage, and a total of 5 stages. Then, the total gain by the PMT will be:
\begin{align}
    G_{tot} = G^5
\end{align}

For the purposes of our proposed experiment, we hope to construct multiple PMT with special requirements. First, we let our PMT release it's output not onto a readout, but let the electrons fly in free space. We also hope it to have a low amplification factor, and construct multiple PMT's with different number of stages. Then, by switching out the PMT, one is able to quantify exactly number of stages that the states collapses at $D_0$. If performed correctly, this will become the first experiment to observe and quantify the collapse of a quantum state! 



